Poisoning Prevention in Federated Learning and Differential Privacy via Stateful Proofs of Execution

The rise in IoT-driven distributed data analytics, coupled with increasing privacy concerns, has led to a demand for effective privacy-preserving and federated data collection/model training mechanisms. In response, approaches such as Federated Learning (FL) and Local Differential Privacy (LDP) have been proposed and attracted much attention over the past few years. However, they still share the common limitation of being vulnerable to poisoning attacks wherein adversaries compromising edge devices feed forged (a.k.a. poisoned) data to aggregation back-ends, undermining the integrity of FL/LDP results. In this work, we propose a system-level approach to remedy this issue based on a novel security notion of Proofs of Stateful Execution (PoSX) for IoT/embedded devices' software. To realize the PoSX concept, we design SLAPP: a System-Level Approach for Poisoning Prevention. SLAPP leverages commodity security features of embedded devices - in particular ARM TrustZoneM security extensions - to verifiably bind raw sensed data to their correct usage as part of FL/LDP edge device routines. As a consequence, it offers robust security guarantees against poisoning. Our evaluation, based on real-world prototypes featuring multiple cryptographic primitives and data collection schemes, showcases SLAPP's security and low overhead.

==> experiment.tex <==
% Instrumentation: 44 bytes - 2 LoC

% FLASH (absolute)
% \acron
% HMAC: 17.5k
% ECC: 35k
% Sphincs: 24.5k
% Baseline
% HMAC: 16972
% ECC: 34476
% Sphincs: 24012

% SAML11 @ 32MHz and 32KB of Non-secure Flash
% Runtime (\acron):
% HMAC: 0.403308629989624 sec
% ECC: 2.5730948448181152 sec
% ED25519: 14.798 sec
% Sphincs: 103.426 sec

% Runtime (Baseline):
% HMAC: 0.39847612380981445 sec
% ECC: 2.569 sec
% ED25519: 14.802 sec
% Sphincs: 103.57 sec


% Mem Usage => Stack used (\acron) + global/static vars = total:
% HMAC: 1392 bytes + 88 = 1480
% ECC: 1324+292 = 1616 
% ED25519: 1356 bytes + 168 = 1524
% ECC: 1324 + 292 = 1616
% Sphincs: 3376 bytes  + 236 = 3612
% Stack used (Baseline):
% HMAC: 1224 bytes + 56 = 1280
% ECC: 1324+260 = 1584 
% ED25519: 1348 bytes + 136 = 1484
% Sphincs: 3376 bytes + 204 = 3580

% Binary Size:
% \acron
% ECC: 28028

% Runtime w.r.t. PMEM size
% x [4KB, 8KB, 12KB, 16KB, 20KB, 24KB, 28KB, 32KB]
% BaselineHMAC = [0.0790095329284668, 0.12446427345275879, 0.17047786712646484, 0.21570920944213867, 0.2619667053222656, 0.30765604972839355, 0.3547205924987793, 0.3993499279022217]

% aronHMAC = [0.08375906944274902, 0.129044771194458, 0.1743919849395752, 0.22248125076293945, 0.26660728454589844, 0.3120884895324707, 0.35889720916748047, 0.4047119617462158]

% acronECC = [2.2518115043640137, 2.2988271713256836, 2.343857526779175, 2.389514923095703, 2.435807228088379, 2.484464645385742, 2.527547597885132, 2.5684518814086914]

% BaselineECC = [2.2474045753479004, 2.28305029869079, 2.33861470222473, 2.3731114864349365, 2.4212682247161865, 2.4771275520324707, 2.52275013923645, 2.5620603561401367]

% BaselineED2519 = [14.5045485496521, 14.547479629516602, 14.592308759689331, 14.636958837509155, 14.68211317062378, 14.725340604782104, 14.77086091041565, 14.814823389053345]

% acronEd25519 = [14.49381399154663, 14.541197299957275, 14.586003541946411, 14.63441801071167, 14.681947469711304, 14.724242925643921, 14.77163815498352, 14.816883087158203]

% BaselineSphincs = [103.38624906539917, 103.37984991073608, 103.84800958633423, 103.65508389472961, 103.63118529319763, 103.55302786827087, 103.58099865913391, 103.62103605270386]

% \acron Sphincs = [103.60318803787231, 103.6840922832489, 103.44010138511658, 103.64500617980957, 103.55301690101624, 103.56300139427185, 103.77327919006348, 103.92214632034302]

% ===================================================================================

% Nucleo
% Runtime (\acron):
% HMAC: 0.6651020050048828 sec
% ECC: 1.0523254871368408 sec
% Sphincs: 20.78967022895813 sec

% Runtime (Baseline):
% HMAC: 0.6641349792480469 sec
% ECC: 1.0513103008270264 sec
% Sphincs: 20.820197820663452 sec

% FLASH size (\acron):
% Everything until __acle_se_SECURE_pox (before HAL_MspInit)
% Unnecessary: 510 => (Error_Handler+__acle_se_SECURE_RegisterCallback+__acle_se_SECURE_send+__acle_se_SECURE_recv+__acle_se_SECURE_avg+)
% HMAC: 4700 - 508 + 500 (isr) = 4692
% ECC: 17944 - 508 + 500 (isr) = 17936
% SPHINCS: 11636 - 508 + 500 (isr) = 11628

% FLASH size (baseline)
% \acron - secure_setState - secure_checkState
% HMAC = 4692 - 356 = 4336
% ECC: 17936 - 356 = 17580
% SPHINCS: 11628 - 356 = 11272

% Mem usage using static analyzer:
% \acron: (static stack analyzer, data, bss, rodata)
% HMAC: 1928 (static stack analyzer) + 0x2c (data) + 0x174 (bss) + 0x18c (rodata) = 2740
% ECC: 1568 + 0xec + 0x2b0 + 0x320 = 3292
% Sphincs: 7888+0xb0+0x184+0x2fc = 9216

% Baseline (static stack analyzer, data, bss, rodata)
% HMAC: 1912 (static stack analyzer) + 0x10 (data) + 0x16c (bss) + 0x18c (rodata) = 2688
% ECC: 1252 + 0xd0 + 0x2b0 + 0x320 = 2948
% Sphincs: 5552 + 0x94 + 0x17c + 0x2fc = 6844

% Mem Usage => Stack+data+bss used (\acron):
% HMAC: 1200 (stack -- [fdf8 to e000] -> Magic Number filled, overwritten [fdf8 to f948]), 0x34 (.data), 0x17c (bss) = 1632
% ECC: 968 (stack -- [fed0 to e000] -> Magic Number filled, overwritten [fed0 to fb08]), 0xf4 (.data), 0x2b8 (.bss) = 1908
% Sphincs: 3040 (stack -- [f608 to e000] -> Magic Number filled, overwritten [f608 to ea28]), 0xb8 (.data), 0x18c (.bss) = 3620

% Stack used (Baseline):
% HMAC: 1192 (stack -- [fe00 to e000] -> Magic Number filled, overwritten [fe00 to f958]), 0x18 (.data), 0x174 (bss) = 1588
% ECC: 808 (stack -- [fed0 to e000] -> Magic Number filled, overwritten [fed0 to fba8]), 0xd8 (data), 0x2b8 (bss) = 1720
% Sphincs: 3040 (stack -- [f608 to e000] -> Magic Number filled, overwritten [f608 to ea28]), 0x9c (data), 0x184 (bss) = 3584

% Runtime w.r.t. PMEM size
% x [0x8000, 0x10000, 0x18000, 0x20000, 0x28000, 0x30000, 0x38000, 0x40000]
% x [32KB, 64KB, 96KB, 128KB, 160KB, 192KB, 224KB, 256KB]

% acronHMAC = [0.08888602256774902, 0.173173189163208, 0.252321720123291, 0.3364126682281494, 0.41768884658813477, 0.5004100799560547, 0.5857069492340088, 0.6651020050048828]

% acronECC = [0.47394752502441406, 0.5569748878479004, 0.6409292221069336, 0.7227809429168701, 0.8042812347412109, 0.8859663009643555, 0.9706435203552246, 1.0523254871368408]

% acronSphinc = [20.22879409790039, 20.314748287200928, 20.415284633636475, 20.489927530288696, 20.583590269088745, 20.65108561515808, 20.711153745651245, 20.78967022895813]

% baselineHMAC = [0.08971309661865234, 0.16980695724487305, 0.25185275077819824, 0.3343665599822998, 0.4167177677154541, 0.5044071674346924, 0.5815010070800781, 0.6641349792480469]

% baselinECC = [0.4726254940032959, 0.5546512603759766, 0.6428525447845459, 0.7209932804107666, 0.8018155097961426, 0.8883063793182373, 0.9678099155426025, 1.0513103008270264]

% baselineSphince = [20.23530149459839, 20.323694467544556, 20.405871391296387, 20.490225076675415, 20.5687735080719, 20.653220653533936, 20.73797035217285, 20.820197820663452]


% ===================================================================================


% Case study:
% FL with 8 neurons and data is collected hourly for 5 days
% FLASH:  Everything until __acle_se_SECURE_pox (before HAL_MspInit)
% Unnecessary: 400 => (Error_Handler+__acle_se_SECURE_RegisterCallback+__acle_se_SECURE_send+__acle_se_SECURE_recv)
% S \acron: 5032(6700) - 400 = 4.632
% NS \acron (everything until Reset_Handler): 45444
% NS Baseline: 1.328
% S Baseline (up until Reset_Handler): 50300
% FL memory: (Setup, Collection, Local Train) => fixed 1392+92=1484
% FL runtime: (Setup, Collection, Local Train) => (0.51, 2.30, 21.84)
% FL NS memory (Setup): 8 (stack) + 3320 (bss+data+rodata) = 3328
% FL NS memory (Collection): 16 (stack) + 3320 (bss+data+rodata)  = 3336
% FL NS memory (Train): 2472 (stack) + 26712 (heap) + 3320 (bss+data+rodata) = 32048
% FL-baseline S memory (Setup): 1976 (stack) + (0x888+0x1a0+0x340) (rodata+data+bss) = 5408
% FL-baseline S memory (Collect): 1976 (stack) + (0x888+0x1a0+0x340) (rodata+data+bss)
% FL-baseline S memory: 1976 (stack) + 26712 (heap) + (0x888+0x1a0+0x340) (rodata+data+bss) = 32120
% FL-baseline NS RAM: 296 (stack) + 0x1d0+0x68+0x27c (rodata+data+bss) = 1500

% end-to-end runtime
% days = [1,5,10,15,20]
% setupRuntime = [.69, .69, .69, .69, .69]
% collectRuntime = [.69, .69*5, .69*10, .69*15, .69*20]
% trainRuntime = [1.92, 3.77, 6.49, 9.22, 11.9]
% total runtime = Setup + Collect * days + Train

% FLASH: absolute
% \acro
% S: 17396
% NS: 57176
% Baseline:
% NS: 7488
% S: 71340

% LDP
% \acron (rodata+data+bss)
% NS: 288+0x23c+0x68+0x6a0 = 2660
% Baseline (stack+rodata+data+bss)
% NS: 288+0x1b0+0x68+0x19c = 1236
% S: 1912+0x2f8+0x68+0x850 = 4904


% end-to-end runtime
% numCollected = [1,5,10,15,20]
% setupRuntime = [.687,.687,.687,.687,.687]
% collectRuntime = [.684,.684*5,.684*10,.684*15,.684*20]



